dPRO: A Generic Profiling and Optimization System for Expediting Distributed DNN Training

Distributed training using multiple devices (e.g., GPUs) has been widely adopted for learning DNN models over large datasets. However, the performance of large-scale distributed training tends to be far from linear speed-up in practice. Given the complexity of distributed systems, it is challenging to identify the root cause(s) of inefficiency and exercise effective performance optimizations when unexpected low training speed occurs. To date, there exists no software tool which diagnoses performance issues and helps expedite distributed DNN training, while the training can be run using different deep learning frameworks. This paper proposes dPRO, a toolkit that includes: (1) an efficient profiler that collects runtime traces of distributed DNN training across multiple frameworks, especially fine-grained communication traces, and constructs global data flow graphs including detailed communication operations for accurate replay; (2) an optimizer that effectively identifies performance bottlenecks and explores optimization strategies (from computation, communication, and memory aspects) for training acceleration. We implement dPRO on multiple deep learning frameworks (TensorFlow, MXNet) and representative communication schemes (AllReduce and Parameter Server). Extensive experiments show that dPRO predicts the performance of distributed training in various settings with < 5% errors in most cases and finds optimization strategies with up to 3.48x speed-up over the baselines.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

% \subsection{Bottleneck Analysis}
% \bpfname{} can also help to identify performance bottlenecks in a distributed DNN training job. The poor performance of distributed training can be caused by many factors, e.g., slow pre-processing or unoptimized operator implementations, we seek to identify the fine-grained bottlenecks so that developers can improve the training systems or DNN models accordingly, e.g., increasing the number of threads for data pre-processing or fusing multiple small GPU kernels. We first find the critical path of the global execution graph and for each node/operator on the critical path, we estimate the iteration time using the trace-based replayer after setting its duration to 0.
% % \Hu{need discussion}. 
% Then we take the top-$k$ operators with the largest reduction of iteration time as the bottleneck. This can give operator developers some inspiration to tell which operators they should focus on to optimize.

==> related_work.tex <==
%-------------------------------------------------------------------------------
\section{Related Work}

\begin{comment}
\mypara{DNN Training Profiler.}
Current mainly used profiling tools in DNN ecosystem can be divided into three categories: 1) Hardware profiling tools. For example, Nvidia provides NVProf \cite{nvprof} to collect the start/end time of each kernel, GPU core utilization and memory usage, as well as plenty of other hardware counters. Nvidia has also developed CUPTI \cite{CUPTI} to enable utilizing these profiling information at runtime. These vendor-provided tools fail to capture dependencies among operators in a DNN model. 2) Framework built-in profiling tool. ML frameworks, like TensorFlow \cite{abadi2016tensorflow}, PyTorch \cite{paszke2019pytorch} and MXNet \cite{chen2015mxnet}, provide their own built-in profilers, which can collect operator or layer level traces. 
% MXNet provides a profiler which can profile the duration of all computation operations executed on GPU. But the time used by MXNet Profiler is relative and the trace names are not unique, i.e., two different operations may share the same name in one iteration. 
% TensorFlow can also utilize CUPTI to collect more fine-grained kernel-level computation traces. But these tools are also aimed at collecting computation traces, so they are not sufficient to analyze distributed DNN training jobs. 
Although there are some distributed APIs in TensorFlow and MXNet, the built-in profiler can still only get coarse-grained communication traces - taking the synchronization of each gradient as a black box; 3) Third-party tools. Some distributed ML frameworks, like BytePS \cite{jiang2020unified} for parameter server architecture and Horovod \cite{horovod2020tensorfusion} for all-reduce, enable to profile communication across multiple devices. But they can only provide coarse-grained communication traces without correlation to computation. %For example, Horovod only collects traces for one "coordinator" GPU and regards a NCCL All-Reduce as a single task. Since a gradient/tensor is divided into multiple chunks to perform All-Reduce across workers. This coarse-grained communication traces are not enough to analyze the detailed behaviour of each partitioned tensor.

Daydream \cite{zhu2020daydream} predicts DNN training performance using kernel-level traces and tracks dependencies by mapping kernel-level traces to corresponding DNN operators. It fails to accurately simulate distributed DNN training jobs because Daydream only uses traces on one GPU to estimate the iteration time of a distributed training job. It estimates communication time theoretically with bandwidth and tensor size, which can not reflect the difference of different all-reduce algorithms and network protocols.

\end{comment}



% \Hu{How to explain BytePS, inaccurate Push/Pull traces}, 

% 3)\textbf{PyTorch Profiler}PyTorch also provides a profiler for computation operations and the trace names are not unique
% TensorFlow Profiler \cite{tensorflowProfiler} can profile execution time of each operators on both GPU and CPU and the profiled traces can be dumped into a timeline. Its Trace Viewer can visualize the timeline and help developers to identify the performance issues. TensorFlow Profiler can also provide high level summary of model performance, including iteration time, memory usage, GPU utilization and most time-consuming operators. Based on these profiling information, TensorFlow Profiler lists some simple recommendations to developers. E.g., if it detect the percentage of 16-bit device computation is too low when running on V100 GPUs, it will suggest to replace more 32-bit computation 16-bit, since V100 GPUs are highly optimized for 16-bit operations with Tensor Cores \cite{markidis2018nvidia};

% FlexFlow \cite{jia2018beyond} introduces an execution simulator for distributed DNN training to help search parallelization strategies. However, it still focus on how to accurately simulate the execution time of DNN operators with different parallelization strategies but use a similar theoretical method to estimate communication time with bandwidth based on coarse-grained communication traces. This simple method is not scalable to different network configurations.

% \Hu{Runtime Performance Prediction for Deep Learning Models with Graph Neural Network}
% machine learning forecast like TVM, operator-level optimization. 

% \textbf{Search Algorithm}
% To accelerate DNN training, many researches about Deep Learning Compiler have been conducted to optimize the structure of DNN model and hardware deployment strategy \cite{chen2018tvm,abadi2016tensorflow}. For example, TVM \cite{chen2018tvm} performs some graph-level optimizations (e.g., operator fusion, data layout transformations) and operator-level optimizations (e.g., memory latency hiding) to achieve considerable performance improvement for deep learning workloads across diverse hardware back-ends. In order to avoid manually searching the best optimization strategy, TVM also collects training data and leverages a ML-based cost model to estimate the performance of tensor operators with different optimization and configurations, then automatically explore and search for the optimized tensor operators. However, this ML-learning based method is time-consuming \Hu{figure out more gaps} \CY{We also use ML based cost model...} and developers actually needs a more systematic method to evaluate the performance improvement and guide them to tune the model structure for diverse physical devices. Therefore, we propose \sysname{} Profiler, which can accurately simulate distributed DNN training runtime based on the fine-grained communication traces.

\mypara{Optimizations of DNN Training.}
% As the DNN model size becomes increasingly large, many work has been proposed to optimize DNN models. 
%\cwu{autoML is not relevant so remove} Some works about Neural Architecture Search (NAS) \cite{elsken2019neural,liu2018progressive,pham2018efficient} aim to search for the optimal DNN model architecture, but they usually require users to program all possible architectures in DNN scripts. AutoML \cite{he2021automl} and Retiarii \cite{zhang2020retiarii} have also been proposed to allow users only providing input data and they will automatically find a DNN architecture based on the NAS algorithm specified by users. However, both NAS and AutoML still focus on single-machine cases and they are mostly used for model inference rather than DNN training.
Besides, operator fusion is a widely applied technique to speed up DNN model computation and is considered in a variety of optimizers and compilers \cite{tensorflowxla, roesch2018relay, zheng2020fusionstitching, zhou2020transferable, sivathanu2019astra}. XLA \cite{tensorflowxla} and TVM Relay \cite{roesch2018relay} use rule-based methods to find operator fusion candidates. FusionStitching \cite{zheng2020fusionstitching} and GO \cite{zhou2020transferable} searches for the optimal fusion strategy using cost models, but does not consider the problem in a distributed setting. %Astra \cite{sivathanu2019astra} is a profiling based approach that can search for GEMM fusion and other optimization strategies during the training process. The authors claim that their methods also work for distributed settings but no detailed discussions or evaluations are given. 
In contrast, \sysname{} aims to explore the trade-off between acceleration brought by fusing operators and the performance degrade caused by the decreased overlap between computation and communication. % We also do not directly search for operator fusion at kernel level, but considers the partitioning of sub-graphs into XLA compiled clusters, since the custom communication operators in BytePS and Horovod follows dependency at cluster level, not individual fused kernels in XLA.

\haibin{Mention memory related optimizations and tools (e.g. memory estimator from MSR)} 
Gist \cite{jain2018gist} further proposes to reduce memory usage from source by encoding intermediate results). vDNN \cite{rhu2016vdnn} (mitigates intermediate results from GPU memory to CPU). 


% \textbf{Tensor Fusion}
% Horovod tensor fusion, two envs to control


% \textbf{Mixed Precision Training}
% From fp32 to fp16, AMP 

% \textbf{Memory Related}
% Recomputing or reduce the batch size.

% \textbf{Deep learning compiler}
% Rammer: Enabling Holistic Deep Learning Compiler Optimizations with rTasks, 

% like BytePS and Horovod



